Harnessing Synthetic Preference Data for Enhancing Temporal Understanding of Video-LLMs

While Video Large Language Models (Video-LLMs) have demonstrated remarkable performance across general video understanding benchmarks-particularly in video captioning and descriptive tasks-they consistently underperform on tasks that require fine-grained temporal understanding. This limitation arises due to the lack of visual complexity and temporal nuance in current fine-tuning datasets, leading these models to rely heavily on language-based reasoning rather than truly understanding video dynamics. In this work, we propose TimeWarp, a systematic method to create a targeted synthetic temporal dataset to fine-tune the model's responses to encourage it to focus on the given input video. We introduce a large-scale preference dataset, created using TimeWarp, that captures intricate temporal dynamics often overlooked, grounding the model's responses to visual and temporal information. We demonstrate that when our method is applied to existing models, it significantly improves performance on temporal understanding benchmarks, highlighting the effectiveness of our proposed datasets in advancing temporal understanding in Video-LLMs, resulting in an absolute improvement in performance across seven benchmarks. Code is available at https://github.com/sameepv21/timewarp.

==> sec/7_limitations_and_future_work.tex <==
\section{Limitations and Future Work}
\label{sec:limitations and future}

While data generated using {\finetune} demonstrates substantial improvements across a variety of benchmarks, some limitations persist that indicate directions for future enhancement. First limitation stems from the use of basic clip captions from FineVideo, which may not fully capture the intricate dynamics between events in a video sequence. By augmenting these captions to include more detailed event transitions and contextual cues, future iterations of {\finetune} could provide richer temporal context, thereby improving the model's ability to discern subtle changes and relationships between scenes. Second, applying {\finetune} to other advanced architectures and SOTA, such as Video-Chat and InternVideo, will reveal further insights into how different model architectures can process and retain temporal information. Such adaptations could also open up opportunities for multi-modal datasets, potentially combining audio and text cues with video to provide a more comprehensive framework for real-world video understanding. However, our method can be extended easily to any other model architecture that can use both SFT and preference fine-tuning.

==> sec/9_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tables/eval_results.tex <==
\begin{table*}[hbt!]\centering
\caption{Performance comparison of current SOTA models with baseline and finetuned models we selected against multiple benchmarks. \textbf{Bold} numbers indicate the best performance and \underline{underlined} numbers denotes the second best performance.}\label{tab:eval_results}
\scriptsize
\scalebox{0.9}{
\begin{tabular}{lccccccccccccc}\toprule
\multirow{2}{*}{\textbf{Models}} &\multirow{2}{*}{\textbf{Perception Test}} &\multirow{2}{*}{\textbf{TVBench}} &\multicolumn{3}{c}{\textbf{VinoGround}} &\multicolumn{2}{c}{\textbf{TempCompass}} &\multicolumn{2}{c}{\textbf{TimeWar}} &\multirow{2}{*}{\textbf{CinePile}} &\multirow{2}{*}{\textbf{MSRVTT}} &\multirow{2}{*}{\textbf{Next-QA}} \\ \cmidrule(lr){4-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
& & &\textbf{Text} &\textbf{Video} &\textbf{Group} &\textbf{MCQs} &\textbf{Cap-Match} &\textbf{Normal} &\textbf{Shuffled} & & & \\
\midrule
Qwen2.5 &64.13 &44.13 &36.2 &27.6 &11.4 &\textbf{71.07} &75.04 &61.12 &55.56 &Ready &Ready &Ready \\
InternVideo & \underline{67.49} & \textbf{50.77} &39.8 & 28.59 & \underline{11.6} &69.41 & \textbf{79.7} & \textbf{66.76} & \textbf{60.44} & Ready & Ready & Ready \\
VideoChat &\textbf{69.14} &\ul{50.59} &\textbf{55.8} &\textbf{33.4} &\textbf{21.8} &\ul{71.01} &\ul{77.11} &\underline{66.1 }&\underline{57.24} &Ready &Ready &Ready \\
LLaVA-OneVision &56.53 &43.57 &39.4 &28.59 &\underline{15} &64.17 &71.98 &55.06 &49.59 &35.13 &Ready &76.07 \\
LLaVA-Hound (SFT) &52.61 &45.24 &24 &26 &6.2 &56.51 &60.1 &49.74 &48.96 &31.53 &67.6 &64.79 \\
Video-LLaMA3 &55.1 &43.57 &31.8 &29.2 &10.2 &63.92 &71.32 &53.9 &51.4 &34.04 &69.59 &69.81 \\
\hdashline
\addlinespace[2pt]
\orange{\textbf{LLaVA-Hound (TimeWarp)}} &\orange{57.57} &\orange{47.39} &\orange{22.2} &\orange{\underline{31.6}} &\orange{6.6} &\orange{61.28} &\orange{60.95} &\orange{55.36} &\orange{55.14} &\orange{32.02} &\orange{78.86} &\orange{55.32} \\
\orange{\textbf{Video-LLaMA3 (TimeWarp)}} &\orange{56.76} &\orange{43.53} &\orange{33.4} &\orange{27.4} &\orange{7.8} &\orange{65.57} &\orange{72.92} &\orange{56.44} &\orange{52.86} &\orange{35.66} &\orange{70.85} &\orange{71.61} \\

\bottomrule
\end{tabular}
}
\end{table*}

==> tables/kto_training_config.tex <==
\begin{table}[h]
\centering
\caption{KTO Training Configuration}
\label{tab:kto_training_config}
\vspace{0.3cm}
\begin{tabular}{ll}
\toprule
\textbf{Parameter} & \textbf{Value} \\
\midrule
Data Samples & 15k \\
Epochs & 3 \\
Training Steps & 1.4k (similar to TimeWarp-DPO: 1.2k) \\
Global Batch Size & 32 (using 2 A100 GPUs) \\
Learning Rate & 5e-7 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/ptest_abstraction.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage{xcolor,colortbl} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{Detailed analysis of Perception Test for Abstract questions across different categories}\label{tab:ptest_abstraction}
\scriptsize
\scalebox{1.3}{
\begin{tabular}{lcccccc}\toprule
\multicolumn{6}{c}{\textbf{Perception Test - Abstraction}} \\\midrule
\textbf{Model Name} &\textbf{Descriptive} &\textbf{Explanatory} &\textbf{Predictive} &\textbf{Counterfactual} &\textbf{Overall} \\
\midrule
LLaVA-OneVision &50.69 &- &37.5 &15.66 &49.56 \\
LLaMA-VID &30.79 &- &35.93 &22.89 &30.91 \\
LLaVA-Next-Video &37.35 &- &37.5 &28.91 &42.84 \\
\midrule
LLaVA-Hound-SFT &49.02 &- &39.45 &38.55 &48.42 \\
LLaVA-Hound-DPOC &47.05 &- &39.84 &\gray{43.37} &46.65 \\
\midrule
LLaVA-Hound-DPO &48.79 &- &36.72 &\green{\textbf{44.58}} &48.17 \\
\hdashline
\addlinespace[2pt]
\orange{LLaVA-Hound-TW (Ours)} &\green{\textbf{52.44}} &- &\green{\textbf{50.39}} &34.94 &\green{\textbf{52.08}} \\
\orange{LLaVA-Hound-TW-3k (Ours)} &\gray{51.74} &- &\gray{45.31} &37.35 &\gray{51.22} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/ptest_memory.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage{xcolor,colortbl} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{Detailed analysis of Perception Test for Memory based questions across different categories}\label{tab:ptest_memory}
\scriptsize
\scalebox{1.3}{
\begin{tabular}{lcccccc}\toprule
\multicolumn{6}{c}{\textbf{Perception Test - Memory}} \\\midrule
\textbf{Model Name} &\textbf{Descriptive} &\textbf{Explanatory} &\textbf{Predictive} &\textbf{Counterfactual} &\textbf{Overall} \\
LLaVA-OneVision &\green{\textbf{44.17}} &\green{\textbf{61.48}} &- &36.11 &\green{\textbf{46.91}} \\
LLaMA-VID &39.13 &28.15 &- &33.33 &36.86 \\
LLaVA-Next-Video &38.08 &\gray{37.77} &- &44.44 &38.33 \\
\midrule
LLaVA-Hound-SFT &42.26 &28.15 &- &\gray{47.22} &39.95 \\
LLaVA-Hound-DPOC &\gray{44.0} &28.15 &- &\green{\textbf{63.89}} &\gray{42.09} \\
\midrule
LLaVA-Hound-DPO &42.43 &27.4 &- &47.22 &39.95 \\
\hdashline
\addlinespace[2pt]
\orange{LLaVA-Hound-TW (Ours)} &38.61 &22.22 &- &38.89 &35.66 \\
\orange{LLaVA-Hound-TW-3k (Ours)} &38.61 &32.59 &- &44.44 &37.81 \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/ptest_physics.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage{xcolor,colortbl} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{Detailed analysis of Perception Test for Physics related questions across different categories}\label{tab:ptest_physics}
\scriptsize
\scalebox{1.3}{
\begin{tabular}{lcccccc}\toprule
\multicolumn{6}{c}{\textbf{Perception Test - Physics}} \\\midrule
\textbf{Model Name} &\textbf{Descriptive} &\textbf{Explanatory} &\textbf{Predictive} &\textbf{Counterfactual} &\textbf{Overall} \\
\midrule
LLaVA-OneVision &52.27 &32.78 &38.9 &41.93 &48.03 \\
LLaMA-VID &34.92 &29.53 &32.11 &9.68 &33.7 \\
LLaVA-Next-Video &47.43 &24.87 &37.59 &35.48 &42.84 \\
\midrule
LLaVA-Hound-SFT &52.8 &41.35 &79.11 &\gray{45.16} &52.19 \\
LLaVA-Hound-DPOC &49.18 &45.11 &57.18 &41.94 &48.86 \\
\midrule
LLaVA-Hound-DPO &53.2 &41.92 &78.59 &45.16 &52.56 \\
\hdashline
\addlinespace[2pt]
\orange{LLaVA-Hound-TW (Ours)} &\green{\textbf{58.62}} &\gray{45.59} &\green{\textbf{81.2}} &\green{\textbf{58.06}} &\green{\textbf{57.5}5} \\
\orange{LLaVA-Hound-TW-3k (Ours)} &\gray{56.14} &\green{\textbf{49.18}} &\gray{79.11} &41.94 &\gray{56.11} \\
\bottomrule
\end{tabular}
}
\end{table*}

==> tables/ptest_semantics.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage{xcolor,colortbl} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{Detailed analysis of Perception Test that target semantic understanding of models across different categories}\label{tab:ptest_semantics}
\scriptsize
\scalebox{1.3}{
\begin{tabular}{lcccccc}\toprule
\multicolumn{6}{c}{\textbf{Perception Test - Semantics}} \\\midrule
\textbf{Model Name} &\textbf{Descriptive} &\textbf{Explanatory} &\textbf{Predictive} &\textbf{Counterfactual} &\textbf{Overall} \\
LLaVA-OneVision &\green{\textbf{80.94}} &48 &- &60.38 &75 \\
LLaMA-VID &42.59 &23.78 &- &31.4 &39.22 \\
LLaVA-Next-Video &\gray{61.71} &27.24 &- &34.29 &42.84 \\
\midrule
LLaVA-Hound-SFT &56.73 &30.92 &- &36.71 &51.94 \\
LLaVA-Hound-DPOC &54.82 &42.81 &- &32.85 &52.14 \\
\midrule
LLaVA-Hound-DPO &56.88 &31.03 &- &38.65 &52.14 \\
\hdashline
\addlinespace[2pt]
\orange{LLaVA-Hound-TW (Ours)} &59.47 &50.81 &- &37.68 &57.33 \\
\orange{LLaVA-Hound-TW-3k (Ours)} &58.13 &68.97 &- &39.61 &59.19 \\
\bottomrule
\end{tabular}
}
\end{table*}
